Head-wise Adaptive Rotary Positional Encoding for Fine-Grained Image Generation

Transformers rely on explicit positional encoding to model structure in data. While Rotary Position Embedding (RoPE) excels in 1D domains, its application to image generation reveals significant limitations such as fine-grained spatial relation modeling, color cues, and object counting. This paper identifies key limitations of standard multi-dimensional RoPE-rigid frequency allocation, axis-wise independence, and uniform head treatment-in capturing the complex structural biases required for fine-grained image generation. We propose HARoPE, a head-wise adaptive extension that inserts a learnable linear transformation parameterized via singular value decomposition (SVD) before the rotary mapping. This lightweight modification enables dynamic frequency reallocation, semantic alignment of rotary planes, and head-specific positional receptive fields while rigorously preserving RoPE's relative-position property. Extensive experiments on class-conditional ImageNet and text-to-image generation (Flux and MMDiT) demonstrate that HARoPE consistently improves performance over strong RoPE baselines and other extensions. The method serves as an effective drop-in replacement, offering a principled and adaptable solution for enhancing positional awareness in transformer-based image generative models.

==> math_commands.tex <==
%%%%% NEW MATH DEFINITIONS %%%%%

\usepackage{amsmath,amsfonts,bm}

% Mark sections of captions for referring to divisions of figures
\newcommand{\figleft}{{\em (Left)}}
\newcommand{\figcenter}{{\em (Center)}}
\newcommand{\figright}{{\em (Right)}}
\newcommand{\figtop}{{\em (Top)}}
\newcommand{\figbottom}{{\em (Bottom)}}
\newcommand{\captiona}{{\em (a)}}
\newcommand{\captionb}{{\em (b)}}
\newcommand{\captionc}{{\em (c)}}
\newcommand{\captiond}{{\em (d)}}

% Highlight a newly defined term
\newcommand{\newterm}[1]{{\bf #1}}


% Figure reference, lower-case.
\def\figref#1{figure~\ref{#1}}
% Figure reference, capital. For start of sentence
\def\Figref#1{Figure~\ref{#1}}
\def\twofigref#1#2{figures \ref{#1} and \ref{#2}}
\def\quadfigref#1#2#3#4{figures \ref{#1}, \ref{#2}, \ref{#3} and \ref{#4}}
% Section reference, lower-case.
\def\secref#1{section~\ref{#1}}
% Section reference, capital.
\def\Secref#1{Section~\ref{#1}}
% Reference to two sections.
\def\twosecrefs#1#2{sections \ref{#1} and \ref{#2}}
% Reference to three sections.
\def\secrefs#1#2#3{sections \ref{#1}, \ref{#2} and \ref{#3}}
% Reference to an equation, lower-case.
\def\eqref#1{equation~\ref{#1}}
% Reference to an equation, upper case
\def\Eqref#1{Equation~\ref{#1}}
% A raw reference to an equation---avoid using if possible
\def\plaineqref#1{\ref{#1}}
% Reference to a chapter, lower-case.
\def\chapref#1{chapter~\ref{#1}}
% Reference to an equation, upper case.
\def\Chapref#1{Chapter~\ref{#1}}
% Reference to a range of chapters
\def\rangechapref#1#2{chapters\ref{#1}--\ref{#2}}
% Reference to an algorithm, lower-case.
\def\algref#1{algorithm~\ref{#1}}
% Reference to an algorithm, upper case.
\def\Algref#1{Algorithm~\ref{#1}}
\def\twoalgref#1#2{algorithms \ref{#1} and \ref{#2}}
\def\Twoalgref#1#2{Algorithms \ref{#1} and \ref{#2}}
% Reference to a part, lower case
\def\partref#1{part~\ref{#1}}
% Reference to a part, upper case
\def\Partref#1{Part~\ref{#1}}
\def\twopartref#1#2{parts \ref{#1} and \ref{#2}}

\def\ceil#1{\lceil #1 \rceil}
\def\floor#1{\lfloor #1 \rfloor}
\def\1{\bm{1}}
\newcommand{\train}{\mathcal{D}}
\newcommand{\valid}{\mathcal{D_{\mathrm{valid}}}}
\newcommand{\test}{\mathcal{D_{\mathrm{test}}}}

\def\eps{{\epsilon}}


% Random variables
\def\reta{{\textnormal{$\eta$}}}
\def\ra{{\textnormal{a}}}
\def\rb{{\textnormal{b}}}
\def\rc{{\textnormal{c}}}
\def\rd{{\textnormal{d}}}
\def\re{{\textnormal{e}}}
\def\rf{{\textnormal{f}}}
\def\rg{{\textnormal{g}}}
\def\rh{{\textnormal{h}}}
\def\ri{{\textnormal{i}}}
\def\rj{{\textnormal{j}}}
\def\rk{{\textnormal{k}}}
\def\rl{{\textnormal{l}}}
% rm is already a command, just don't name any random variables m
\def\rn{{\textnormal{n}}}
\def\ro{{\textnormal{o}}}
\def\rp{{\textnormal{p}}}
\def\rq{{\textnormal{q}}}
\def\rr{{\textnormal{r}}}
\def\rs{{\textnormal{s}}}
\def\rt{{\textnormal{t}}}
\def\ru{{\textnormal{u}}}
\def\rv{{\textnormal{v}}}
\def\rw{{\textnormal{w}}}
\def\rx{{\textnormal{x}}}
\def\ry{{\textnormal{y}}}
\def\rz{{\textnormal{z}}}

% Random vectors
\def\rvepsilon{{\mathbf{\epsilon}}}
\def\rvtheta{{\mathbf{\theta}}}
\def\rva{{\mathbf{a}}}
\def\rvb{{\mathbf{b}}}
\def\rvc{{\mathbf{c}}}
\def\rvd{{\mathbf{d}}}
\def\rve{{\mathbf{e}}}
\def\rvf{{\mathbf{f}}}
\def\rvg{{\mathbf{g}}}
\def\rvh{{\mathbf{h}}}
\def\rvu{{\mathbf{i}}}
\def\rvj{{\mathbf{j}}}
\def\rvk{{\mathbf{k}}}
\def\rvl{{\mathbf{l}}}
\def\rvm{{\mathbf{m}}}
\def\rvn{{\mathbf{n}}}
\def\rvo{{\mathbf{o}}}
\def\rvp{{\mathbf{p}}}
\def\rvq{{\mathbf{q}}}
\def\rvr{{\mathbf{r}}}
\def\rvs{{\mathbf{s}}}
\def\rvt{{\mathbf{t}}}
\def\rvu{{\mathbf{u}}}
\def\rvv{{\mathbf{v}}}
\def\rvw{{\mathbf{w}}}
\def\rvx{{\mathbf{x}}}
\def\rvy{{\mathbf{y}}}
\def\rvz{{\mathbf{z}}}

% Elements of random vectors
\def\erva{{\textnormal{a}}}
\def\ervb{{\textnormal{b}}}
\def\ervc{{\textnormal{c}}}
\def\ervd{{\textnormal{d}}}
\def\erve{{\textnormal{e}}}
\def\ervf{{\textnormal{f}}}
\def\ervg{{\textnormal{g}}}
\def\ervh{{\textnormal{h}}}
\def\ervi{{\textnormal{i}}}
\def\ervj{{\textnormal{j}}}
\def\ervk{{\textnormal{k}}}
\def\ervl{{\textnormal{l}}}
\def\ervm{{\textnormal{m}}}
\def\ervn{{\textnormal{n}}}
\def\ervo{{\textnormal{o}}}
\def\ervp{{\textnormal{p}}}
\def\ervq{{\textnormal{q}}}
\def\ervr{{\textnormal{r}}}
\def\ervs{{\textnormal{s}}}
\def\ervt{{\textnormal{t}}}
\def\ervu{{\textnormal{u}}}
\def\ervv{{\textnormal{v}}}
\def\ervw{{\textnormal{w}}}
\def\ervx{{\textnormal{x}}}
\def\ervy{{\textnormal{y}}}
\def\ervz{{\textnormal{z}}}

% Random matrices
\def\rmA{{\mathbf{A}}}
\def\rmB{{\mathbf{B}}}
\def\rmC{{\mathbf{C}}}
\def\rmD{{\mathbf{D}}}
\def\rmE{{\mathbf{E}}}
\def\rmF{{\mathbf{F}}}
\def\rmG{{\mathbf{G}}}
\def\rmH{{\mathbf{H}}}
\def\rmI{{\mathbf{I}}}
\def\rmJ{{\mathbf{J}}}
\def\rmK{{\mathbf{K}}}
\def\rmL{{\mathbf{L}}}
\def\rmM{{\mathbf{M}}}
\def\rmN{{\mathbf{N}}}
\def\rmO{{\mathbf{O}}}
\def\rmP{{\mathbf{P}}}
\def\rmQ{{\mathbf{Q}}}
\def\rmR{{\mathbf{R}}}
\def\rmS{{\mathbf{S}}}
\def\rmT{{\mathbf{T}}}
\def\rmU{{\mathbf{U}}}
\def\rmV{{\mathbf{V}}}
\def\rmW{{\mathbf{W}}}
\def\rmX{{\mathbf{X}}}
\def\rmY{{\mathbf{Y}}}
\def\rmZ{{\mathbf{Z}}}

% Elements of random matrices
\def\ermA{{\textnormal{A}}}
\def\ermB{{\textnormal{B}}}
\def\ermC{{\textnormal{C}}}
\def\ermD{{\textnormal{D}}}
\def\ermE{{\textnormal{E}}}
\def\ermF{{\textnormal{F}}}
\def\ermG{{\textnormal{G}}}
\def\ermH{{\textnormal{H}}}
\def\ermI{{\textnormal{I}}}
\def\ermJ{{\textnormal{J}}}
\def\ermK{{\textnormal{K}}}
\def\ermL{{\textnormal{L}}}
\def\ermM{{\textnormal{M}}}
\def\ermN{{\textnormal{N}}}
\def\ermO{{\textnormal{O}}}
\def\ermP{{\textnormal{P}}}
\def\ermQ{{\textnormal{Q}}}
\def\ermR{{\textnormal{R}}}
\def\ermS{{\textnormal{S}}}
\def\ermT{{\textnormal{T}}}
\def\ermU{{\textnormal{U}}}
\def\ermV{{\textnormal{V}}}
\def\ermW{{\textnormal{W}}}
\def\ermX{{\textnormal{X}}}
\def\ermY{{\textnormal{Y}}}
\def\ermZ{{\textnormal{Z}}}

% Vectors
\def\vzero{{\bm{0}}}
\def\vone{{\bm{1}}}
\def\vmu{{\bm{\mu}}}
\def\vtheta{{\bm{\theta}}}
\def\va{{\bm{a}}}
\def\vb{{\bm{b}}}
\def\vc{{\bm{c}}}
\def\vd{{\bm{d}}}
\def\ve{{\bm{e}}}
\def\vf{{\bm{f}}}
\def\vg{{\bm{g}}}
\def\vh{{\bm{h}}}
\def\vi{{\bm{i}}}
\def\vj{{\bm{j}}}
\def\vk{{\bm{k}}}
\def\vl{{\bm{l}}}
\def\vm{{\bm{m}}}
\def\vn{{\bm{n}}}
\def\vo{{\bm{o}}}
\def\vp{{\bm{p}}}
\def\vq{{\bm{q}}}
\def\vr{{\bm{r}}}
\def\vs{{\bm{s}}}
\def\vt{{\bm{t}}}
\def\vu{{\bm{u}}}
\def\vv{{\bm{v}}}
\def\vw{{\bm{w}}}
\def\vx{{\bm{x}}}
\def\vy{{\bm{y}}}
\def\vz{{\bm{z}}}

% Elements of vectors
\def\evalpha{{\alpha}}
\def\evbeta{{\beta}}
\def\evepsilon{{\epsilon}}
\def\evlambda{{\lambda}}
\def\evomega{{\omega}}
\def\evmu{{\mu}}
\def\evpsi{{\psi}}
\def\evsigma{{\sigma}}
\def\evtheta{{\theta}}
\def\eva{{a}}
\def\evb{{b}}
\def\evc{{c}}
\def\evd{{d}}
\def\eve{{e}}
\def\evf{{f}}
\def\evg{{g}}
\def\evh{{h}}
\def\evi{{i}}
\def\evj{{j}}
\def\evk{{k}}
\def\evl{{l}}
\def\evm{{m}}
\def\evn{{n}}
\def\evo{{o}}
\def\evp{{p}}
\def\evq{{q}}
\def\evr{{r}}
\def\evs{{s}}
\def\evt{{t}}
\def\evu{{u}}
\def\evv{{v}}
\def\evw{{w}}
\def\evx{{x}}
\def\evy{{y}}
\def\evz{{z}}

% Matrix
\def\mA{{\bm{A}}}
\def\mB{{\bm{B}}}
\def\mC{{\bm{C}}}
\def\mD{{\bm{D}}}
\def\mE{{\bm{E}}}
\def\mF{{\bm{F}}}
\def\mG{{\bm{G}}}
\def\mH{{\bm{H}}}
\def\mI{{\bm{I}}}
\def\mJ{{\bm{J}}}
\def\mK{{\bm{K}}}
\def\mL{{\bm{L}}}
\def\mM{{\bm{M}}}
\def\mN{{\bm{N}}}
\def\mO{{\bm{O}}}
\def\mP{{\bm{P}}}
\def\mQ{{\bm{Q}}}
\def\mR{{\bm{R}}}
\def\mS{{\bm{S}}}
\def\mT{{\bm{T}}}
\def\mU{{\bm{U}}}
\def\mV{{\bm{V}}}
\def\mW{{\bm{W}}}
\def\mX{{\bm{X}}}
\def\mY{{\bm{Y}}}
\def\mZ{{\bm{Z}}}
\def\mBeta{{\bm{\beta}}}
\def\mPhi{{\bm{\Phi}}}
\def\mLambda{{\bm{\Lambda}}}
\def\mSigma{{\bm{\Sigma}}}

% Tensor
\DeclareMathAlphabet{\mathsfit}{\encodingdefault}{\sfdefault}{m}{sl}
\SetMathAlphabet{\mathsfit}{bold}{\encodingdefault}{\sfdefault}{bx}{n}
\newcommand{\tens}[1]{\bm{\mathsfit{#1}}}
\def\tA{{\tens{A}}}
\def\tB{{\tens{B}}}
\def\tC{{\tens{C}}}
\def\tD{{\tens{D}}}
\def\tE{{\tens{E}}}
\def\tF{{\tens{F}}}
\def\tG{{\tens{G}}}
\def\tH{{\tens{H}}}
\def\tI{{\tens{I}}}
\def\tJ{{\tens{J}}}
\def\tK{{\tens{K}}}
\def\tL{{\tens{L}}}
\def\tM{{\tens{M}}}
\def\tN{{\tens{N}}}
\def\tO{{\tens{O}}}
\def\tP{{\tens{P}}}
\def\tQ{{\tens{Q}}}
\def\tR{{\tens{R}}}
\def\tS{{\tens{S}}}
\def\tT{{\tens{T}}}
\def\tU{{\tens{U}}}
\def\tV{{\tens{V}}}
\def\tW{{\tens{W}}}
\def\tX{{\tens{X}}}
\def\tY{{\tens{Y}}}
\def\tZ{{\tens{Z}}}


% Graph
\def\gA{{\mathcal{A}}}
\def\gB{{\mathcal{B}}}
\def\gC{{\mathcal{C}}}
\def\gD{{\mathcal{D}}}
\def\gE{{\mathcal{E}}}
\def\gF{{\mathcal{F}}}
\def\gG{{\mathcal{G}}}
\def\gH{{\mathcal{H}}}
\def\gI{{\mathcal{I}}}
\def\gJ{{\mathcal{J}}}
\def\gK{{\mathcal{K}}}
\def\gL{{\mathcal{L}}}
\def\gM{{\mathcal{M}}}
\def\gN{{\mathcal{N}}}
\def\gO{{\mathcal{O}}}
\def\gP{{\mathcal{P}}}
\def\gQ{{\mathcal{Q}}}
\def\gR{{\mathcal{R}}}
\def\gS{{\mathcal{S}}}
\def\gT{{\mathcal{T}}}
\def\gU{{\mathcal{U}}}
\def\gV{{\mathcal{V}}}
\def\gW{{\mathcal{W}}}
\def\gX{{\mathcal{X}}}
\def\gY{{\mathcal{Y}}}
\def\gZ{{\mathcal{Z}}}

% Sets
\def\sA{{\mathbb{A}}}
\def\sB{{\mathbb{B}}}
\def\sC{{\mathbb{C}}}
\def\sD{{\mathbb{D}}}
% Don't use a set called E, because this would be the same as our symbol
% for expectation.
\def\sF{{\mathbb{F}}}
\def\sG{{\mathbb{G}}}
\def\sH{{\mathbb{H}}}
\def\sI{{\mathbb{I}}}
\def\sJ{{\mathbb{J}}}
\def\sK{{\mathbb{K}}}
\def\sL{{\mathbb{L}}}
\def\sM{{\mathbb{M}}}
\def\sN{{\mathbb{N}}}
\def\sO{{\mathbb{O}}}
\def\sP{{\mathbb{P}}}
\def\sQ{{\mathbb{Q}}}
\def\sR{{\mathbb{R}}}
\def\sS{{\mathbb{S}}}
\def\sT{{\mathbb{T}}}
\def\sU{{\mathbb{U}}}
\def\sV{{\mathbb{V}}}
\def\sW{{\mathbb{W}}}
\def\sX{{\mathbb{X}}}
\def\sY{{\mathbb{Y}}}
\def\sZ{{\mathbb{Z}}}

% Entries of a matrix
\def\emLambda{{\Lambda}}
\def\emA{{A}}
\def\emB{{B}}
\def\emC{{C}}
\def\emD{{D}}
\def\emE{{E}}
\def\emF{{F}}
\def\emG{{G}}
\def\emH{{H}}
\def\emI{{I}}
\def\emJ{{J}}
\def\emK{{K}}
\def\emL{{L}}
\def\emM{{M}}
\def\emN{{N}}
\def\emO{{O}}
\def\emP{{P}}
\def\emQ{{Q}}
\def\emR{{R}}
\def\emS{{S}}
\def\emT{{T}}
\def\emU{{U}}
\def\emV{{V}}
\def\emW{{W}}
\def\emX{{X}}
\def\emY{{Y}}
\def\emZ{{Z}}
\def\emSigma{{\Sigma}}

% entries of a tensor
% Same font as tensor, without \bm wrapper
\newcommand{\etens}[1]{\mathsfit{#1}}
\def\etLambda{{\etens{\Lambda}}}
\def\etA{{\etens{A}}}
\def\etB{{\etens{B}}}
\def\etC{{\etens{C}}}
\def\etD{{\etens{D}}}
\def\etE{{\etens{E}}}
\def\etF{{\etens{F}}}
\def\etG{{\etens{G}}}
\def\etH{{\etens{H}}}
\def\etI{{\etens{I}}}
\def\etJ{{\etens{J}}}
\def\etK{{\etens{K}}}
\def\etL{{\etens{L}}}
\def\etM{{\etens{M}}}
\def\etN{{\etens{N}}}
\def\etO{{\etens{O}}}
\def\etP{{\etens{P}}}
\def\etQ{{\etens{Q}}}
\def\etR{{\etens{R}}}
\def\etS{{\etens{S}}}
\def\etT{{\etens{T}}}
\def\etU{{\etens{U}}}
\def\etV{{\etens{V}}}
\def\etW{{\etens{W}}}
\def\etX{{\etens{X}}}
\def\etY{{\etens{Y}}}
\def\etZ{{\etens{Z}}}

% The true underlying data generating distribution
\newcommand{\pdata}{p_{\rm{data}}}
% The empirical distribution defined by the training set
\newcommand{\ptrain}{\hat{p}_{\rm{data}}}
\newcommand{\Ptrain}{\hat{P}_{\rm{data}}}
% The model distribution
\newcommand{\pmodel}{p_{\rm{model}}}
\newcommand{\Pmodel}{P_{\rm{model}}}
\newcommand{\ptildemodel}{\tilde{p}_{\rm{model}}}
% Stochastic autoencoder distributions
\newcommand{\pencode}{p_{\rm{encoder}}}
\newcommand{\pdecode}{p_{\rm{decoder}}}
\newcommand{\precons}{p_{\rm{reconstruct}}}

\newcommand{\laplace}{\mathrm{Laplace}} % Laplace distribution

\newcommand{\E}{\mathbb{E}}
\newcommand{\Ls}{\mathcal{L}}
\newcommand{\R}{\mathbb{R}}
\newcommand{\emp}{\tilde{p}}
\newcommand{\lr}{\alpha}
\newcommand{\reg}{\lambda}
\newcommand{\rect}{\mathrm{rectifier}}
\newcommand{\softmax}{\mathrm{softmax}}
\newcommand{\sigmoid}{\sigma}
\newcommand{\softplus}{\zeta}
\newcommand{\KL}{D_{\mathrm{KL}}}
\newcommand{\Var}{\mathrm{Var}}
\newcommand{\standarderror}{\mathrm{SE}}
\newcommand{\Cov}{\mathrm{Cov}}
% Wolfram Mathworld says $L^2$ is for function spaces and $\ell^2$ is for vectors
% But then they seem to use $L^2$ for vectors throughout the site, and so does
% wikipedia.
\newcommand{\normlzero}{L^0}
\newcommand{\normlone}{L^1}
\newcommand{\normltwo}{L^2}
\newcommand{\normlp}{L^p}
\newcommand{\normmax}{L^\infty}

\newcommand{\parents}{Pa} % See usage in notation.tex. Chosen to match Daphne's book.

\DeclareMathOperator*{\argmax}{arg\,max}
\DeclareMathOperator*{\argmin}{arg\,min}

\DeclareMathOperator{\sign}{sign}
\DeclareMathOperator{\Tr}{Tr}
\let\ab\allowbreak


==> method_full.tex <==
\section{Methodology}
\subsection{Preliminary of RoPE}
In a vector space, each dimension or combination of dimensions essentially corresponds to a direction of information. In the attention Q/K space, a query vector $q$ can be expressed as a linear combination of certain ``semantic basis vectors'':
\[
q = \alpha_1 d_1 + \alpha_2 d_2 + \cdots + \alpha_r d_r
\]
where $d_i$ represents an ``information direction'', and $\alpha_i$ denotes the strength in this direction.\\
RoPE essentially performs rotation:
\[q' = R_m q, \quad k' = R_n k\]
Rotation is a two-dimensional plane operation. This means RoPE assumes that certain dimensions form pairs to create a ``directional plane,'' and then encodes relative positional information by rotating in this plane.RoPE does not uniformly inject positional information into all directions, but rather confines it to a set of predefined directional planes.\\
The matrix Q serves as a learnable basis transformation that realigns the originally scattered "semantic directions" in the high-dimensional space to the rotational blocks of RoPE. 
\[ \tilde{q} = R_m (Q q), \quad \tilde{k} = R_n (Q k)\]
Rather than "mechanically applying rotations to every dimension," RoPE "selectively injects positional information only into the semantic directions that truly require it."\
\Different semantic directions perceive positional information differently; thus, through Q, the allocation of frequencies corresponding to different semantic directions can also be learned.
\paragraph{Formulation of 2D RoPE.}
The Rotary Position Embedding (RoPE) is to achieve relative position encoding through absolute position encoding.In one dimension, its form is as follows.
{\scriptsize
\begin{equation}
q'=R_m q = 
\left(
\begin{array}{ccccccc}
\cos m\theta_0 & \sin m\theta_0 & & &  \\
-\sin m\theta_0 & \cos m\theta_0 & & & & \\
& & \cos m\theta_1 & \sin m\theta_1 & & \\
& & -\sin m\theta_1 & \cos m\theta_1 & & \\
 & & & \ddots &\ddots &\ddots & \\
& & & & & \cos m\theta_{d/2-1}&\sin m\theta_{d/2-1} \\
& & & & & -\sin m\theta_{d/2-1}&\cos m\theta_{d/2-1} \\
\end{array}
\right)
\left(
\begin{array}{c}
q_0 \\
q_1 \\
q_2 \\
q_3 \\
\vdots \\
q_{d-2} \\
q_{d-1} \\
\end{array}
\right)
\end{equation}}
Where $\theta$ is the frequency factor, typically defined as:
\begin{equation}
\theta_i = 10000^{-2i/d}, \quad \text{for } i = 0,1,\ldots,d/2-1 \label{eq:theta}
\end{equation}
The implementation is achieved by constructing a rotation matrix and applying it to q and k.In other words, when it multiplies the vector $q$ at position $m$ by matrix $R_m$, and the vector $k$ at position $n$ by matrix $R_n$, then use the transformed $q'$ and $k'$ sequences to compute Attention, Attention will automatically incorporate relative position information. This is because the following identity holds:
\begin{equation}
(R_m q)^\top (R_n k) = 
q^\top R_m^\top R_n k= 
q^\top R_{n-m} k
\end{equation}
\begin{equation}
(R_m Qq)^\top (R_n Qk) = 
q^\top Q^\top R_m^\top R_n Qk= 
q^\top Q^\top R_{n-m} Qk
\end{equation}
And it commonly used form of 2D RoPE is as follows.
{\scriptsize
\begin{equation}
q' = R_{(x,y)} q =
\left(
\begin{array}{cccccccccc}
\cos \theta_{0}x & -\sin \theta_{0}x & \cdots & 0 & 0 & 0 & 0 & \cdots & 0 & 0 \\
\sin \theta_{0}x & \cos \theta_{0}x  & \cdots & 0 & 0 & 0 & 0 & \cdots & 0 & 0 \\
\vdots           & \vdots            & \ddots & \vdots & \vdots & \vdots & \vdots & \cdots & 0 & 0 \\
0 & 0 & \cdots & \cos \theta_{d/4-1}x & -\sin \theta_{d/4-1}x & 0 & 0 & \cdots & 0 & 0 \\
0 & 0 & \cdots & \sin \theta_{d/4-1}x &  \cos \theta_{d/4-1}x & 0 & 0 & \cdots & 0 & 0 \\
0 & 0 & \cdots & 0 & 0 & \cos \theta_{0}y & -\sin \theta_{0}y & \cdots & 0 & 0 \\
0 & 0 & \cdots & 0 & 0 & \sin \theta_{0}y &  \cos \theta_{0}y & \cdots & 0 & 0 \\
\vdots & \vdots & \vdots & \vdots & \vdots & \vdots & \vdots & \ddots & \vdots & \vdots \\
0 & 0 & \cdots & 0 & 0 & 0 & 0 & \cdots & \cos \theta_{d/4-1}y & -\sin \theta_{d/4-1}y \\
0 & 0 & \cdots & 0 & 0 & 0 & 0 & \cdots & \sin \theta_{d/4-1}y &  \cos \theta_{d/4-1}y
\end{array}
\right)
\left(
\begin{array}{c}
q_0 \\
q_1 \\
q_2 \\
q_3 \\
q_4 \\
q_5 \\
q_6 \\
q_7 \\
\vdots \\
q_{d-2} \\
q_{d-1} \\
\end{array}
\right)
\end{equation}
}
In the 2D case, is also satisfies:
\begin{equation}
(R_{(x_1,y_1)} q)^\top (R_{(x_2,y_2)} k) = 
q^\top R_{(x_1,y_1)}^\top R_{(x_2,y_2)} k= 
q^\top R_{(x_1-x_2,y_1-y_2)} k
\end{equation}

\paragraph{Potential Problems in 2D RoPE.}
Both 1D RoPE and 2D RoPE share the same mathematical operation:
In the vector space of $q$ and $k$, certain dimensions are grouped into pairs (forming 2D subspaces), and within each subspace, a complex-form rotation is applied — that is, the 2D vector is multiplied by a rotation matrix.This way, every dimension of the $q$ and $k$ vectors carries positional information. However,in 2D RoPE, each dimension carries positional information for only one direction, because in the rotation matrix, each rotation angle is determined solely by either $x$ or $y$.\\
We partition the vectors and rotation matrices into two blocks.
\begin{equation}
    q = \begin{bmatrix} q_1 \\ q_2 \end{bmatrix}, \quad
    k = \begin{bmatrix} k_1 \\ k_2 \end{bmatrix},\quad
    R(x_i, y_i) =
    \begin{bmatrix}
    R_x(x_i) & 0 \\
    0 & R_y(y_i)
    \end{bmatrix}
\end{equation}
where $q_1$ and $k_1$ correspond to the x-related components and $q_2$ and $k_2$ correspond to the y-related components.And $R_x(x_i)$ and $R_y(y_i)$ are orthogonal rotation matrices determined solely by $x_i$ and $y_i$, respectively.
Applying the rotation to $q$ and $k$ yields:
\[
q_i' = R(x_i, y_i)\, q =
\begin{bmatrix}
R_x(x_i) q_1 \\
R_y(y_i) q_2
\end{bmatrix}, \quad
k_j' = R(x_j, y_j)\, k =
\begin{bmatrix}
R_x(x_j) k_1 \\
R_y(y_j) k_2
\end{bmatrix}.
\]
This shows that $R_x(x_i) q_1$ contains only the positional information from $x_i$, and $R_y(y_i) q_2$ contains only the information from $y_i$. The same applies to $k$.\\The attention mechanism computes the similarity between positions $i$ and $j$ as:
\[
q_i'^\top k_j' =
\begin{bmatrix}
q_1^\top R_x(x_i)^\top  q_2^\top R_y(y_i)^\top
\end{bmatrix}
\begin{bmatrix}
R_x(x_j) k_1 \\
R_y(y_j) k_2
\end{bmatrix}.
\]
Expanding this, we obtain:
\[
q_i'^\top k_j' =
q_1^\top \big(R_x(x_i)^\top R_x(x_j)\big) k_1
+
q_2^\top \big(R_y(y_i)^\top R_y(y_j)\big) k_2.
\]
The first term depends only on $x_i, x_j$ (and $q_1, k_1$), representing the x-direction contribution.
The second term depends only on $y_i, y_j$ (and $q_2, k_2$), representing the y-direction contribution.
Thus, the inner product is the sum of the x and y contributions.\\
This summation operation compresses the two-dimensional positional information into a single scalar, effectively performing a dimensionality reduction on the global 2D relative positional information. Although the scalar can represent the overall positional information, the independent contributions from the x and y directions are merged, and the full structural relationships of the 2D positional information cannot be preserved.\textbf{The overall positional information is not equivalent to the global positional information.}



\subsection{Current Methods}
To address the problem in the original 2D-RoPE where the full two-dimensional positional information cannot be preserved in high-dimensional space—the dimensionality reduction effect,some methods have been proposed .
\paragraph{STRING} STRING models interactions between spatial dimensions by introducing learnable parameters.The details are as follows:
\[
R(\mathbf{r}_i) = \exp \left( \sum_{k=1}^{d_c} \mathbf{L}_k [\mathbf{r}_i]_k \right),
\]
where $\{\mathbf{L}_k\}_{k=1}^{d_c} \subset \mathbb{R}^{d \times d}$ is a set of learnable and commuting skew-symmetric generators,$d_c$ is the number of spatial dimensions, and $d$ is the feature dimension. Given a set of queries or keys $\{\mathbf{z}_i\}_{i=1}^N \subset \mathbb{R}^d$ at positions $\{\mathbf{r}_i\}_{i=1}^N \subset \mathbb{R}^{d_c}$, where $N$ is the number os tokens ,their positions are encoded as:
\[
\mathbf{z}_i \to R(\mathbf{r}_i) \mathbf{z}_i \quad \forall i \in \{1, \dots, N\}.
\]
Although STRING learns matrices $\{\mathbf{L}_k\}$ to model inter-dimensional interactions, it may violate RoPE's injective mapping property: $\mathbf{r}_i \neq \mathbf{r}_j \nRightarrow R(\mathbf{r}_i) \neq R(\mathbf{r}_j)$.
\paragraph{Rethinking RoPE}
To model inter-dimensional interactions while maintaining RoPE's injective mapping property,Rethinking RoPE uses a global orthogonal matrix $Q$ apply linear combinations across all dimensions of a rotation matrix. Mathematically, if the original rotation matrix is
\[
R(x, y) = \mathrm{diag}\big(R_x(x), R_y(y)\big),
\]
then, introducing the orthogonal matrix $Q$, a similarity transformation gives
\[
R'(x, y) = Q R(x, y) Q^\top.
\]
To illustrate the structure of high-dimensional rotation matrices under \textbf{Rethinking RoPE}, we consider a 8-dimensional vector (four pairs of 2D rotation planes) as an example.
The 8D rotation matrix can be block-diagonalized along $x$ and $y$ dimensions:
\[
R = \text{diag}\big(R_2(x\theta_1), R_2(x\theta_2), R_2(y\theta_1), R_2(y\theta_2)\big)
\]
which expands to:
\[
R = 
\begin{bmatrix}
\cos x\theta_1 & -\sin x\theta_1 & 0 & 0 & 0 & 0 & 0 & 0 \\
\sin x\theta_1 & \cos x\theta_1 & 0 & 0 & 0 & 0 & 0 & 0 \\
0 & 0 & \cos x\theta_2 & -\sin x\theta_2 & 0 & 0 & 0 & 0 \\
0 & 0 & \sin x\theta_2 & \cos x\theta_2 & 0 & 0 & 0 & 0 \\
0 & 0 & 0 & 0 & \cos y\theta_1 & -\sin y\theta_1 & 0 & 0 \\
0 & 0 & 0 & 0 & \sin y\theta_1 & \cos y\theta_1 & 0 & 0 \\
0 & 0 & 0 & 0 & 0 & 0 & \cos y\theta_1 & -\sin y\theta_1 \\
0 & 0 & 0 & 0 & 0 & 0 & \sin y\theta_1 & \cos y\theta_1
\end{bmatrix}
\]
where each $R_2(\theta_i)$ represents a 2D rotation matrix:
\[
R_2(x(y)\theta_i) = 
\begin{bmatrix}
\cos x(y)\theta_i & -\sin x(y)\theta_i \\
\sin x(y)\theta_i & \cos x(y)\theta_i
\end{bmatrix}
\]
To achieve Full-Dimensional Mixing, we introduce a general 8×8 orthogonal matrix $Q$, which mixes all dimensions across different rotation planes:
\[
Q = 
\begin{bmatrix}
q_{11} & q_{12} & \cdots & q_{18} \\
q_{21} & q_{22} & \cdots & q_{28} \\
\vdots & \vdots & \ddots & \vdots \\
q_{81} & q_{82} & \cdots & q_{88}
\end{bmatrix},
\quad Q^\top Q = I
\]
% \[
% Q =
% \begin{bmatrix}
% c & 0 & -s & 0 \\
% 0 & c & 0 & -s \\
% s & 0 & c & 0 \\
% 0 & s & 0 & c
% \end{bmatrix}, \quad
% c = \cos\gamma, \; s = \sin\gamma,
% \]
% The mixed high-dimensional rotation matrix is obtained by similarity transformation:
% \[
% R'(x,y) =
% \begin{bmatrix}
% c^2 \cos\theta_x + s^2 \cos\theta_y & -c^2 \sin\theta_x - s^2 \sin\theta_y & cs(\cos\theta_y - \cos\theta_x) & -cs(\sin\theta_y - \sin\theta_x) \\
% c^2 \sin\theta_x + s^2 \sin\theta_y & c^2 \cos\theta_x + s^2 \cos\theta_y & cs(\sin\theta_y - \sin\theta_x) & cs(\cos\theta_y - \cos\theta_x) \\
% cs(\cos\theta_x - \cos\theta_y) & -cs(\sin\theta_x - \sin\theta_y) & s^2 \cos\theta_x + c^2 \cos\theta_y & -s^2 \sin\theta_x - c^2 \sin\theta_y \\
% cs(\sin\theta_x - \sin\theta_y) & cs(\cos\theta_x - \cos\theta_y) & s^2 \sin\theta_x + c^2 \sin\theta_y & s^2 \cos\theta_x + c^2 \cos\theta_y
% \end{bmatrix}.
% \]
For any $a,b \in \{0,\ldots,7\}$, we have:
\[
R'_{ab} = (QRQ^\top)_{ab} = \sum_{k=0}^3 \sum_{i=0}^1 \sum_{j=0}^1 Q_{a,2k+i}\, R_{2k+i,\, 2k+j}\, Q_{b,2k+j}.
\]
Using the form of each $2\times2$ block $R_{2}(x(y)\theta_k) = \begin{bmatrix}
x(y)c_k & -x(y)s_k \\
x(y)s_k & x(y)c_k
\end{bmatrix}$, where $c_k \equiv \cos\theta_k$ and $s_k \equiv \sin\theta_k$, this simplifies to:
\[
R'_{ab} = \sum_{k=0}^3 \Bigl[ x(y) c_k \bigl(Q_{a,2k}Q_{b,2k} + Q_{a,2k+1}Q_{b,2k+1}\bigr) + x(y) s_k \bigl(Q_{a,2k+1}Q_{b,2k} - Q_{a,2k}Q_{b,2k+1}\bigr) \Bigr].
\]
However, this method still has significant issues. It performs linear combinations of each dimension in the rotation matrix, which disrupt the original two-dimensional sub-rotations within the rotation matrix.Specifically,The key to RoPE lies in the fact that the original rotation matrix $R(\mathbf{r})$ is in a block-diagonal form:
\[
R = \text{diag}\big(R_2(x\theta_1), R_2(x\theta_2), R_2(y\theta_1), R_2(y\theta_2)\big)
\]
where each $R_2(\theta_i)$ represents a 2D rotation matrix,and each $R_2(\theta_i)$ is a pure rotation in a specific two-dimensional plane:
\[
R_2(x(y)\theta_i) = 
\begin{bmatrix}
\cos x(y)\theta_i & -\sin x(y)\theta_i \\
\sin x(y)\theta_i & \cos x(y)\theta_i
\end{bmatrix}
\]
This structure guarantees that:
\[
\|R_2(\theta_i) v\|_2 = \|v\|_2, \\
\angle\left(R_2(\theta_i) u, R_2(\theta_i) v \right) = \angle\left( u,v \right).
\]
That is to say, within each two-dimensional rotational plane, RoPE preserves both the norm and the relative angle. Consequently, the positional information can be represented by a single phase variable $\theta$.\\
However,since $Q$ mixes the coordinates from different two-dimensional planes, the original block structure is destroyed.
\[
R'(x, y) = Q R(x, y) Q^\top.
\]
Consequently, for a specific two-dimensional plane:
\[
\|R'_2 v\|_2 \neq \|v\|_2, \\
\angle\left(R'_2 u, R'_2 v \right) \neq \angle\left( u,v \right).
\]
This disrupts the independence of the two-dimensional rotational blocks,causing (1) the RoPE matrix to lose both its 2D rotation plane interpretability and (2) the original RoPE's phase information structure, which may potentially affect its positional encoding capability.The positional information can not be represented by a single phase variable $\theta$
\subsection{Full-Plane Mixing}
Therefore, we introduce a hybrid approach: Full-Plane Mixing. This method achieves linear combinations between different planes while preserving the rotational structure within each two-dimensional plane. Compared to Full-Dimensional Mixing, Full-Plane Mixing imposes constraints on the pairwise rotations within each two-dimensional plane, thereby avoiding arbitrary linear combinations across all dimensions and only performing mixing between planes.\\
The implementation involves replacing the general rotation matrix \( Q \) with a Kronecker block structure:
\[
Q = G \otimes I_2,
\]
where \( G \in \mathrm{SO}(m) \) is an orthogonal matrix operating on the plane-index space, and \( I_2 \) is the \( 2 \times 2 \) identity matrix. This ensures that the rotational structure within each 2D plane remains unchanged while enabling linear combinations across different planes, thereby achieving Full-Plane Mixing.To illustrate the structure of high-dimensional rotation matrices under Full-Plane Mixing, we also consider a 8-dimensional vector (four pairs of 2D rotation planes) as an example.\\
Let \( G \in \mathrm{SO}(4) \) be a \( 4 \times 4 \) orthogonal matrix:
\[
G = 
\begin{bmatrix}
g_{11} & g_{12} & g_{13} & g_{14} \\
g_{21} & g_{22} & g_{23} & g_{24} \\
g_{31} & g_{32} & g_{33} & g_{34} \\
g_{41} & g_{42} & g_{43} & g_{44}
\end{bmatrix}.
\]
The Kronecker product:
\[
Q = G \otimes I_2 = 
\begin{bmatrix}
g_{11}I_2 & g_{12}I_2 & g_{13}I_2 & g_{14}I_2 \\
g_{21}I_2 & g_{22}I_2 & g_{23}I_2 & g_{24}I_2 \\
g_{31}I_2 & g_{32}I_2 & g_{33}I_2 & g_{34}I_2 \\
g_{41}I_2 & g_{42}I_2 & g_{43}I_2 & g_{44}I_2
\end{bmatrix}_{8 \times 8}.
\]
Through orthogonal transformation:
\[
R' = Q R Q^\top = (G \otimes I_2) \, R \, (G \otimes I_2)^\top
\]
The element-wise formula:
\[
R'(2i-1:2i,\, 2j-1:2j) = \sum_{k=1}^4 g_{ik} g_{jk} R_2(x(y)\theta_k), \quad i,j=1,2,3,4
\]
The $(i,j)$-th block's value is a linear combination of the original four 2D rotation matrices $R_2(x(y)\theta_k)$, 
with coefficients given by $g_{ik}g_{jk}$.
\subsection{Learnable Index Scaling}
Learnable Index Scaling = Learnable $\theta$ base
\subsection{Different Head,Different Setting}

